PRISM: A Promptable and Robust Interactive Segmentation Model with Visual Prompts

In this paper, we present PRISM, a Promptable and Robust Interactive Segmentation Model, aiming for precise segmentation of 3D medical images. PRISM accepts various visual inputs, including points, boxes, and scribbles as sparse prompts, as well as masks as dense prompts. Specifically, PRISM is designed with four principles to achieve robustness: (1) Iterative learning. The model produces segmentations by using visual prompts from previous iterations to achieve progressive improvement. (2) Confidence learning. PRISM employs multiple segmentation heads per input image, each generating a continuous map and a confidence score to optimize predictions. (3) Corrective learning. Following each segmentation iteration, PRISM employs a shallow corrective refinement network to reassign mislabeled voxels. (4) Hybrid design. PRISM integrates hybrid encoders to better capture both the local and global information. Comprehensive validation of PRISM is conducted using four public datasets for tumor segmentation in the colon, pancreas, liver, and kidney, highlighting challenges caused by anatomical variations and ambiguous boundaries in accurate tumor identification. Compared to state-of-the-art methods, both with and without prompt engineering, PRISM significantly improves performance, achieving results that are close to human levels. The code is publicly available at https://github.com/MedICL-VU/PRISM.

==> backup_idea.tex <==
\section{Introduction}
Recently, deep learning-based methods have achieved state-of-the-art performance in various segmentation tasks \cite{isensee2021nnu}. However, achieving robust outcomes remains a challenge due to significant anatomical variations among individuals and ambiguous boundaries in medical images. Alternatively, interactive segmentation models,
such as the segment anything model (SAM) \cite{kirillov2023segment},
offer a solution by involving humans in the loop and utilizing their expertise to achieve precise segmentation. This requires users to indicate
the target region by providing visual prompts, such as points \cite{liu2023simpleclick,kirillov2023segment,luo2021mideepseg,gong20233dsam,li2023promise,wang2018deepigeos,gao2023desam}, boxes \cite{wei2023medsam,zhang2023segment,deng2023sam,wang2018interactive,kirillov2023segment,ma2024segment,chen2023ma,yao2023false},
scribbles \cite{wang2018deepigeos,chen2023scribbleseg,wong2023scribbleprompt,cho2021deepscribble}, and masks \cite{kirillov2023segment,sun2023cfr,wang2023sam,cheng2023sam,liu2023simpleclick}. 
% Furthermore, the desirable interactive segmentation model should be both \underline{effective} \textit{and} \underline{efficient} in responding to these visual prompts given by users for robust segmentation with minimal interactions. 
Furthermore, the robust interactive segmentation model should be \underline{effective}
% both \underline{effective} \textit{and} \underline{efficient} 
in responding to these visual prompts given by users with minimal interactions. 



\textbf{Effective.} Inspired by SAM \cite{kirillov2023segment}, many interactive segmentation methods have been proposed in medical imaging% \cite{ma2024segment,chen2023ma,cheng2023sam,wong2023scribbleprompt,wang2023sam}
. However, most of these SAM-based methods are limited to using a single type of visual prompt \cite{wei2023medsam,gong20233dsam,yao2023false,gao2023desam,li2023promise,deng2023sam,ma2024segment,chen2023ma,zhang2023segment}. This limitation can lead to insufficient information being available, resulting in suboptimal performance that fails to meet effectiveness criteria. 
Due to the heterogeneity in anatomy and appearance of medical images, the models should leverage the advantages of different visuals to achieve optimal performance across various medical applications.
% \xxx{so i think this next part about human-in-loop is either identical to or at least closely related to active learning. no? so im hesitant about the claim at the end of the paragraph that nobody does this. i think maybe you mean nobody does this with sam? we can talk about how to phrase it at the lab mtg. btw i dont think you mentioned sam yet and you really should in the first paragraph}
Moreover, these interactive methods do not involve humans in the loop \cite{gong20233dsam,gao2023desam,zhang2023segment,li2023promise,deng2023sam,wei2023medsam,ma2024segment,chen2023ma,yao2023false}, i.e., the visual prompts are applied to the automatic segmentation model only once, which may not be sufficient to achieve robust outcomes with the initial prompts provided. In contrast, practical applications often necessitate iterative corrections based on new prompts from the user until the outcome meets their criteria \cite{sofiiuk2021reviving}. Unfortunately, few studies have explored this human-in-loop approach for medical interactive segmentation \cite{cheng2023sam,wang2023sam}, and their performance has been suboptimal.

% \textbf{Efficient.} Recent works freeze the encoder weights of SAM and employ additional layers for parameter-efficient fine-tuning. \cite{gao2023desam,wei2023medsam,cheng2023sam,gong20233dsam,li2023promise,chen2023ma}. However, these methods require adherence to the settings of SAM for optimal performance, including upsampling the input image to maintain the same image dimensions as SAM \cite{gong20233dsam,li2023promise,cheng2023sam}, which introduces additional, undesired computational burdens. Importantly, the limited number of tunable parameters in the added layer may indicate more prompts are needed to improve performance, yet the improvements remain marginal across different prompt numbers \cite{gong20233dsam,li2023promise}. In contrast, training a model from scratch with extensive datasets \cite{cheng2023sam,wong2023scribbleprompt,ma2024segment,wang2023sam} improves their overall representational capabilities. However, this approach is time-consuming and typically requires substantial computational resources for optimal performance. Furthermore, models may lack specificity for particular applications due to existing domain gaps in medical imaging \cite{wang2023sam}. This requires an increased number of prompts to reach the required level of task performance. Moreover, 2D models \cite{cheng2023sam,wong2023scribbleprompt,ma2024segment} are not considered ``efficient'' for 3D images as they require significant user effort to provide visual prompts for each slice.











% Moreover, relying solely on a vision transformer encoder may not be optimal for medical image segmentation, as it struggles to capture the detailed information within the images \cite{li2023promise}.


In this work, we aim to present a robust baseline method that balances an effective model with efficiency in user input, for interactive segmentation in medical imaging. Our goal is to strive for human-level performance, as a well-designed human-in-loop segmentation model utilizing visual prompts should gradually improve its results until the outcomes closely match inter-rater variability \cite{haarburger2020radiomics}.




We present PRISM, a \textbf{P}romptable and \textbf{R}obust \textbf{I}nteractive \textbf{S}egmentation \textbf{M}odel, which accepts 
various visual prompts. Our main contributions are:
\begin{itemize}
     \item We leverage an iterative learning \cite{kirillov2023segment,sun2023cfr} and sampling strategy \cite{sofiiuk2021reviving} to train PRISM to achieve continual improvements with each iteration.
     
    \item In each iteration, multiple segmentation masks and their confidence scores are generated \cite{li2018interactive}, selecting the highest score to improve model robustness. This approach is similar to model ensembling but more \xxx{efficient} \cite{linmans2023predictive}
    
     \item We leverage an iterative learning \cite{kirillov2023segment,sun2023cfr} and sampling strategy \cite{sofiiuk2021reviving} to train PRISM to achieve continual improvements with each iteration.

    \item  Moreover, inspired from \cite{jang2019interactive}, the output is fed into a shallow corrective refinement network to correct the mislabeled voxels and refine the final prediction, adhering to the principle of being ``effective and efficient''.

    \item Importantly, a hybrid image encoder with parallel convolutional and transformer paths \cite{li2022cats} is used as the backbone to better capture the local and global information from a medical image.

    \item We evaluated the proposed PRISM on four public datasets for challenging tumor segmentation, including colon \cite{antonelli2022medical}, pancreas \cite{antonelli2022medical}, liver \cite{bilic2023liver} and kidney tumor \cite{heller2021state}, where the anatomical differences among individuals and ambiguous boundaries are present. Comprehensive validation is performed against state-of-the-art automatic and interactive medical image segmentation methods, and PRISM significantly outperforms all of them with substantial improvements.
     
\end{itemize}




\clearpage














==> table/point_table.tex <==
\begin{table*}[t]
\caption{Point prompt number analysis on ``-basic'', where ``-50'' indicates that 50 point prompts are used during training, and ``-ds'' denotes dynamic sampling.}
\label{point table}

\begin{center}
    \begin{tabular}{ l  | c |c |c |c}
    \toprule
    % \hline
    Points & 1 & 10 & 50 &  100\\

    \hline
    -basic &   76.40  & 77.7 &    &   \\
    -basic-50 &  61.30  & 82.41  &  89.92  &  91.30 \\
    -basic-ds &   76.66  & 83.85  & 89.36   & 90.26  \\

    \hline     
     
  \end{tabular} 
\end{center}
\end{table*}






